Sparse Hodge Preference Optimization: Fine-Tuning Language Models toward Alignment beyond Transitive Preferences

The growing adoption of Direct Preference Optimization (DPO), which leverages pairwise preference data, reflects its great success in fine-tuning large language models to align with human expectations. It directly optimizes the policy from human preferences without explicit reward modeling or the complexities of reinforcement learning-based approaches. However, the classic DPO relies on the Bradley--Terry sampling model and cannot effectively capture intransitivity or cyclic structures in aggregated human preference data. In this article, we propose Sparse Hodge Preference Optimization (SHPO), a preference optimization algorithm that augments DPO with a sparse antisymmetric curl residual motivated by the combinatorial Hodge decomposition. We prove that SHPO strictly enlarges DPO's hypothesis class on comparison graphs containing at least one triangle, under some mild regularity conditions on the response representations. We further establish a theoretical guarantee for $\ell_1$-regularized estimation of the curl coefficients under fixed policy and representations. Qualitative studies on three preference datasets under the same QLoRA budget, SHPO-aligned LLM achieves satisfactory performances in preference accuracy, cyclic structure recovery, and GPT-4o-judged generation quality.

==> main-refs.tex <==
% shortcut: cross-document reference numbers are fixed for this submission; regenerate after editing either document.
\newlabel{sec:introduction}{{I}{1}{}{}{}}
\newlabel{fig:overview of SHPO}{{1}{2}{}{}{}}
\newlabel{sec:background}{{II}{2}{}{}{}}
\newlabel{subsec:edge-flow}{{\mbox  {II-A}}{2}{}{}{}}
\newlabel{eq:zero_tria_case}{{1}{3}{}{}{}}
\newlabel{subsec:dpo-gradient-flow}{{\mbox  {II-B}}{3}{}{}{}}
\newlabel{subsec:structural-gap}{{\mbox  {II-C}}{3}{}{}{}}
\newlabel{sec:formulation}{{III}{3}{}{}{}}
\newlabel{sec:method}{{III}{3}{}{}{}}
\newlabel{sec:hodge-decomposition}{{\mbox  {III-A}}{3}{}{}{}}
\newlabel{eq:hodge}{{2}{4}{}{}{}}
\newlabel{rem:hodge-orthogonal}{{1}{4}{}{}{}}
\newlabel{sec:sparse-curl}{{\mbox  {III-B}}{4}{}{}{}}
\newlabel{prop:canonical-skew}{{III.1}{4}{}{}{}}
\newlabel{eq:J}{{3}{4}{}{}{}}
\newlabel{eq:curl}{{4}{4}{}{}{}}
\newlabel{eq:curl_expand}{{5}{4}{}{}{}}
\newlabel{rem:hodge-scope}{{3}{4}{}{}{}}
\newlabel{rem:param-cost}{{4}{4}{}{}{}}
\newlabel{sec:shpo-objective}{{\mbox  {III-C}}{4}{}{}{}}
\newlabel{eq:logit}{{6}{4}{}{}{}}
\newlabel{eq:shpo}{{7}{4}{}{}{}}
\newlabel{eq:shpo-emp}{{8}{5}{}{}{}}
\newlabel{sec:computational details}{{\mbox  {III-D}}{5}{}{}{}}
\newlabel{sec:theoretical-properties}{{IV}{5}{}{}{}}
\newlabel{cor:dpo-special}{{IV.1}{5}{}{}{}}
\newlabel{lem:realizability}{{IV.2}{5}{}{}{}}
\newlabel{thm:strict-inclusion}{{IV.3}{6}{}{}{}}
\newlabel{prop:sparse}{{IV.4}{6}{}{}{}}
\newlabel{sec:experiments}{{V}{7}{}{}{}}
\newlabel{sec:experimental-setup}{{\mbox  {V-A}}{7}{}{}{}}
\newlabel{sec:main-results}{{\mbox  {V-B}}{7}{}{}{}}
\newlabel{sec:ablation-studies}{{\mbox  {V-C}}{7}{}{}{}}
\newlabel{tab:main-results}{{1}{8}{}{}{}}
\newlabel{fig:ablation}{{2}{8}{}{}{}}
\newlabel{fig:sensitivity}{{3}{9}{}{}{}}
\newlabel{fig:sparsity}{{4}{9}{}{}{}}
\newlabel{sec:generation-eval}{{\mbox  {V-E}}{9}{}{}{}}
\newlabel{tab:generation}{{2}{10}{}{}{}}

